Eccentricity Spectra and Integral Eigenvalues of Zero Divisor Graphs

In this work, we study the eccentricity spectra of zero divisor graphs (ZDGs) associated with the ring $\mathbb{Z}_n.$ While previous studies have examined the Laplacian and distance Laplacian spectra of ZDGs, the eccentricity spectra have remained largely unknown due to the unique features of the eccentricity matrix. More specifically, we prove that for a prime $p$, the ZDG and extended ZDG of $\mathbb{Z}_{p^t}$ have integral eccentricity eigenvalues for $t \geq 3$ and $t \geq 2$, respectively. We also find the eccentricity spectra for specific classes of ZDGs and the relationship between the eccentricity matrix of these ZDGs and their tree structures using matrix analysis tools. In addition, for the usefulness of the energy gap in applications, we have calculated the eccentricity energy gap of ZDGs. These findings reveal interesting behaviours of the eccentricity matrix and may contribute to a more profound understanding of the structural properties of ZDGs.

==> ArXiv.bbl.tex <==
\begin{thebibliography}{10}

\bibitem{compare}
Jianfeng Wang, Mei Lu, Lu~Lu, and Francesco Belardo.
\newblock Spectral properties of the eccentricity matrix of graphs.
\newblock {\em Discrete Applied Mathematics}, 279:168--177, 2020.

\bibitem{11}
Milan Randic.
\newblock Dmax--matrix of dominant distances in a graph.
\newblock {\em MATCH Commun. Math. Comput. Chem.}, 70(1):221--238, 2013.

\bibitem{frequency}
R~Radha and N~Mohamed Rilwan.
\newblock Frequency assignment model of zero divisor graph.
\newblock {\em Journal of Applied Mathematics}, 2021:1--8, 2021.

\bibitem{ANDERSON}
David~F. Anderson and Philip~S. Livingston.
\newblock The zero-divisor graph of a commutative ring.
\newblock {\em Journal of Algebra}, 217(2):434--447, 1999.

\bibitem{Bennis}
Driss Bennis, Jilali Mikram, and Fouad Taraza.
\newblock On the extended zero divisor graph of commutative rings.
\newblock {\em Turkish Journal of Mathematics}, 40(2):376--388, 2016.

\bibitem{SR1}
JiMing Guo.
\newblock The laplacian spectral radii of unicyclic and bicyclic graphs with n
  vertices and k pendant vertices.
\newblock {\em Science China Mathematics}, 53:2135--2142, 2010.

\bibitem{SR2}
J~Li, WC~Shiu, Wai~Hong Chan, and A~Chang.
\newblock On the spectral radius of graphs with connectivity at most k.
\newblock {\em Journal of mathematical chemistry}, 46(2):340--346, 2009.

\bibitem{SR3}
Michael Tait and Josh Tobin.
\newblock Three conjectures in extremal spectral graph theory.
\newblock {\em Journal of Combinatorial Theory, Series B}, 126:137--161, 2017.

\bibitem{young}
Matthew Young.
\newblock Adjacency matrices of zero-divisor graphs of integers modulo n.
\newblock {\em Involve, a Journal of Mathematics}, 8(5):753--761, 2015.

\bibitem{magi}
PM~Magi, Sr~Magie Jose, and Anjaly Kishore.
\newblock Spectrum of the zero-divisor graph on the ring of integers modulo n.
\newblock {\em J. Math. Comput. Sci.}, 10(5):1643--1666, 2020.

\bibitem{chat}
Sriparna Chattopadhyay, Kamal~Lochan Patra, and Binod~Kumar Sahoo.
\newblock Laplacian eigenvalues of the zero divisor graph of the ring zn.
\newblock {\em Linear Algebra and its Applications}, 584:267--286, 2020.

\bibitem{pirzada}
S~Pirzada, Bilal~A Rather, M~Aijaz, and TA~Chishti.
\newblock On distance signless laplacian spectrum of graphs and spectrum of
  zero divisor graphs of $\mathbb{Z}_n$.
\newblock {\em Linear and Multilinear Algebra}, 70(17):3354--3369, 2022.

\bibitem{patil}
Avinash Patil and Kiran Shinde.
\newblock Spectrum of the zero-divisor graph of von neumann regular rings.
\newblock {\em Journal of Algebra and Its Applications}, 21(10):2250193, 2022.

\bibitem{bajaj}
Saraswati Bajaj and Pratima Panigrahi.
\newblock On the adjacency spectrum of zero divisor graph of ring $\mathbb{Z}_n$.
\newblock {\em Journal of Algebra and Its Applications}, 21(10):2250197, 2022.

\bibitem{survey}
Dragi{\v{s}}a Cvetkovi{\'c} and Peter Rowlinson.
\newblock The largest eigenvalue of a graph: A survey.
\newblock {\em Linear and multilinear algebra}, 28(1-2):3--33, 1990.

\bibitem{monograph}
Dragan Stevanovi{\^a}c.
\newblock {\em Spectral radius of graphs}.
\newblock Springer, 2015.

\bibitem{La1}
Frank Harary and Allen~J Schwenk.
\newblock Which graphs have integral spectra?
\newblock In {\em Graphs and Combinatorics: Proceedings of the Capital
  Conference on Graph Theory and Combinatorics at the George Washington
  University June 18--22, 1973}, pages 45--51. Springer, 1974.

\bibitem{La2}
Steve Kirkland.
\newblock Constructably laplacian integral graphs.
\newblock {\em Linear algebra and its applications}, 423(1):3--21, 2007.

\bibitem{La3}
Wasin So.
\newblock Rank one perturbation and its application to the laplacian spectrum
  of a graph.
\newblock {\em Linear and Multilinear Algebra}, 46(3):193--198, 1999.

\bibitem{hanlon}
Phil Hanlon.
\newblock Some remarkable combinatorial matrices.
\newblock {\em Journal of Combinatorial Theory, Series A}, 59(2):218--239,
  1992.

\bibitem{von}
Tatjana von Rosen and Dietrich von Rosen.
\newblock On a class of singular nonsymmetric matrices with nonnegative integer
  spectra.
\newblock {\em Algebraic Methods in Statistics and Probability II},
  516:319--325, 2010.

\bibitem{diestel}
Reinhard Diestel.
\newblock {\em Graph theory}.
\newblock Springer (print edition); Reinhard Diestel (eBooks), 2024.

\bibitem{cormen}
Thomas~H Cormen, Charles~E Leiserson, Ronald~L Rivest, and Clifford Stein.
\newblock Introduction to algorithms. mit press and mcgraw-hill.
\newblock 2009.

\bibitem{felsenstein}
J~Felsenstein.
\newblock Inferring phylogenies sinauer associates inc.
\newblock {\em Sunderland, MA. xx+. pp}, 2004.

\bibitem{wanganti}
Jianfeng Wang, Mei Lu, Francesco Belardo, and Milan Randi{\'c}.
\newblock The anti-adjacency matrix of a graph: Eccentricity matrix.
\newblock {\em Discrete Applied Mathematics}, 251:299--309, 2018.

\bibitem{comzero}
Sandra Spiroff and Cameron Wickham.
\newblock A zero divisor graph determined by equivalence classes of zero
  divisors.
\newblock {\em Communications in Algebra}, 39(7):2338--2348, 2011.

\bibitem{bapat}
Ravindra~B Bapat.
\newblock {\em Graphs and matrices}, volume~27.
\newblock Springer, 2010.

\bibitem{cardoso}
Domingos~M Cardoso, Maria Aguieiras~A de~Freitas, Enide~Andrade Martins, and
  Mar{\'\i}a Robbiano.
\newblock Spectra of graphs obtained by a generalization of the join graph
  operation.
\newblock {\em Discrete Mathematics}, 313(5):733--741, 2013.

\bibitem{cardosodistance}
Domingos~M Cardoso, Roberto~C D{\'\i}az, and Oscar Rojo.
\newblock Distance matrices on the h-join of graphs: a general result and
  applications.
\newblock {\em Linear Algebra and its Applications}, 559:34--53, 2018.

\bibitem{perron}
S~Unnikrishna Pillai, Torsten Suel, and Seunghun Cha.
\newblock The perron-frobenius theorem: some of its applications.
\newblock {\em IEEE Signal Processing Magazine}, 22(2):62--75, 2005.

\bibitem{signless}
Shariefuddin Pirzada, Bilal Rather, Rezwan~Ul Shaban, and S~Merajuddin.
\newblock On signless laplacian spectrum of the zero divisor graphs of the ring
  $\mathbb{Z}_n$.
\newblock {\em Korean Journal of Mathematics}, 29(1):13--24, 2021.

\bibitem{wang}
Jianfeng Wang, Mei Lu, Francesco Belardo, and Milan Randi{\'c}.
\newblock The anti-adjacency matrix of a graph: Eccentricity matrix.
\newblock {\em Discrete Applied Mathematics}, 251:299--309, 2018.

\bibitem{mahato}
Iswar Mahato, R~Gurusamy, M~Rajesh Kannan, and S~Arockiaraj.
\newblock Spectra of eccentricity matrices of graphs.
\newblock {\em Discrete Applied Mathematics}, 285:252--260, 2020.

\bibitem{he}
Xiaocong He and Lu~Lu.
\newblock On the largest and least eigenvalues of eccentricity matrix of trees.
\newblock {\em Discrete Mathematics}, 345(1):112662, 2022.

\bibitem{arti}
S~Akbari and A~Mohammadian.
\newblock Zero-divisor graphs of non-commutative rings.
\newblock {\em Journal of Algebra}, 296(2):462--479, 2006.

\bibitem{solution}
Wei Wei, Xiaocong He, and Shuchao Li.
\newblock Solutions for two conjectures on the eigenvalues of the eccentricity
  matrix, and beyond.
\newblock {\em Discrete Mathematics}, 343(8):111925, 2020.

\bibitem{reducible}
Jianfeng Wang, Mei Lu, Francesco Belardo, and Milan Randi{\'c}.
\newblock The anti-adjacency matrix of a graph: Eccentricity matrix.
\newblock {\em Discrete Applied Mathematics}, 251:299--309, 2018.

\bibitem{adja}
Yaokun Wu and Aiping Deng.
\newblock Hoffman polynomials of nonnegative irreducible matrices and strongly
  connected digraphs.
\newblock {\em Linear algebra and its applications}, 414(1):138--171, 2006.

\bibitem{brouwer}
Andries~E Brouwer and Willem~H Haemers.
\newblock {\em Spectra of graphs}.
\newblock Springer Science \& Business Media, 2011.

\bibitem{machineLearn}
Zheng Li, Noushin Omidvar, Wei~Shan Chin, Esther Robb, Amanda Morris, Luke
  Achenie, and Hongliang Xin.
\newblock Machine-learning energy gaps of porphyrins with molecular graph
  representations.
\newblock {\em The Journal of Physical Chemistry A}, 122(18):4571--4578, 2018.

\bibitem{niki}
V~Nikiforov.
\newblock Remarks on the energy of regular graphs.
\newblock {\em Linear Algebra and its Applications}, 508:133--145, 2016.

\bibitem{unionG}
Sasmita Barik, Deabajit Kalita, Sukanta Pati, and Gopinath Sahoo.
\newblock Spectra of graphs resulting from various graph operations and
  products: a survey.
\newblock {\em Special Matrices}, 6(1):323--342, 2018.

\end{thebibliography}

